Backtracking (the) Algorithms on the Hamiltonian Cycle Problem

Even though the Hamiltonian cycle problem is NP-complete, many of its problem instances aren't. In fact, almost all the hard instances reside in one area: near the Koml\'os-Szemer\'edi bound, of $\frac{1}{2}\ v\cdot ln(v) + \frac{1}{2}\ v\cdot ln( ln(v))$ edges, where randomly generated graphs have an approximate 50\% chance of being Hamiltonian. If the number of edges is either much higher or much lower, the problem is not hard -- most backtracking algorithms decide such instances in (near) polynomial time. Recently however, targeted search efforts have identified very hard Hamiltonian cycle problem instances very far away from the Koml\'os-Szemer\'edi bound. In that study, the used backtracking algorithm was Vandegriend-Culberson's, which was supposedly the most efficient of all Hamiltonian backtracking algorithms. In this paper, we make a unified large scale quantitative comparison for the best known backtracking algorithms described between 1877 and 2016. We confirm the suspicion that the Koml\'os-Szemer\'edi bound is a hard area for all backtracking algorithms, but also that Vandegriend-Culberson is indeed the most efficient algorithm, when expressed in consumed computing time. When measured in recursive effectiveness however, the algorithm by Frank Rubin, almost half a century old, performs best. In a more general algorithmic assessment, we conjecture that edge pruning and non-Hamiltonicity checks might be largely responsible for these recursive savings. When expressed in system time however, denser problem instances require much more time per recursion. This is most likely due to the costliness of the extra search pruning procedures, which are relatively elaborate. We supply large amounts of experimental data, and a unified single-program implementation for all six algorithms. All data and algorithmic source code is made public for further use by our colleagues.

==> weggeknipt.tex <==

%uit main.tex: \usepackage{hyperref}

%uitbibtemplate.tex: \usepackage[bookmarks={false},colorlinks={false},hyperref={false}]{hyperref}

abbreviated to \textbf{Cetal's algorithm}

Koekoek\cite{bellman1962dynamic}.

Cheeseman's research
Depth-first strategies

\section{The Hamiltonian Phase Transition}

\section{Acknowledgements}
Many thanks to Richard Karp, Edward Reingold, Andreas Bj\"orklund and Joseph Culberson for answering questions over email.


\section{Geparkeerde stukken tekst}

The hardest instances for \textbf{Cetal's algorithm} are graphs of $v$ vertices that have $\frac{1}{2}(v-1)(v-2)$ edges and consist of a single disconnected vertex and a fully connected clique of size $v-1$. By design, Cetal's algorithm starts at the highest-degree vertex which lies inside the clique from which the backtracking procedure constantly \textit{almost} finds a Hamiltonian cycle. It persistently recurses to almost-maximum search tree depth while branching along almost-maximum degree on every vertex before terminating at a "no solution" answer. The larger the $v$, the closer the algorithm approaches its complexity, or worst-case runtime, of $O(v!)$.

The likeliness of such graphs in the space of possibilities can be calculated (from ˜\cite{erdos1960evolution} or ˜\cite{HopcroftKannan2014DataScience}). The probability of a zero-degree vertex in graph with $v$ vertices and $\frac{1}{2}(v-1)(v-2)$ edges is

\begin{equation} 
N_i = \frac{a}{b}(c \cdot d).
\end{equation}

It turns out these graphs are nearly non-existent in our data with probabilities of $2.8 \cdot 10ˆ{-14}$ for 16-vertex graphs, and $1.5 \cdot 10ˆ{-25}$ and $4.7 \cdot 10ˆ{-38}$ for 24 and 32 edges. This means that even if these hardest graph force Cetal's algorithm ever closer to the worst-case runtime of $O(v!)$, the probability of such graph existing decreases so much faster that hopelidoppie.

\section{Results}
\begin{figure*}[htbp]
%\begin{figure*}[!tb]
\centering%
\includegraphics[width=\linewidth]{results_distri_iter.png} 
%\fbox{\texttt{Insert figure stuff here.}}
\caption{Caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption caption .}\label{figpham}
\end{figure*}



@misc{videoATSP1,
  author = {van den Berg, Daan},
  title = {Video showing where Cetal's results on ATSP are flawed (part1)},
  year = {2020},
  publisher = {YouTube},
  howpublished = {\url{https://www.youtube.com/watch?v=zfqmiLkbCRc}}
}


@misc{videoATSP2,
  author = {van den Berg, Daan},
  title = {Video showing where Cetal's results on ATSP are flawed (part2)},
  year = {2020},
  publisher = {YouTube},
  howpublished = {\url{https://www.youtube.com/watch?v=l8W_GVzqDnk}}
}


@misc{dashed,
  author = {Markus Kr{\"o}tzsch},
  title = {Complexity Theory, Lecture 6: Nondeterministic Polynomial Time},
  year = {2019},
  publisher = {Technische Universit{\"a}t Dresden},
  howpublished = {\url{https://iccl.inf.tu-dresden.de/w/images/0/08/CT2019-Lecture-06-overlay.pdf}}
}

@misc{sourcecodejoeri,
  author = {Sleegers, Joeri},
  title = {Source Code},
  year = {2020},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/Joeri1324/What-s-Difficult-About-the-Hamilton-Cycle-Poblem-}}
}

@misc{Gijsinteractivesite,
  author = {van Horn, Gijs},
  title = {Interactively viewable Hamiltonian Cycle Hardness},
  year = {2020},
  howpublished = {\url{https://hamiltoncycle.gijsvanhorn.nl/}},
}

